Multiparty Sessions based on Proof Nets

We interpret Linear Logic Proof Nets in a term language based on Solos calculus. The system includes a synchronisation mechanism, obtained by a conservative extension of the logic, that enables to define non-deterministic behaviours and multiparty sessions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Alastair F. Donaldson, Vasco Vasconcelos (Eds.): Proceedings\\ of the 7th Workshop on Programming Language Approaches\\ to Concurrency and Communication-cEntric Software (PLACES 2014)\\
EPTCS 155, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.155.1}{10.4204/EPTCS.155.1}}
\pdfoutput=1

